Reconciling High Accuracy, Cost-Efficiency, and Low Latency of Inference Serving Systems

The use of machine learning (ML) inference for various applications is growing drastically. ML inference services engage with users directly, requiring fast and accurate responses. Moreover, these services face dynamic workloads of requests, imposing changes in their computing resources. Failing to right-size computing resources results in either latency service level objectives (SLOs) violations or wasted computing resources. Adapting to dynamic workloads considering all the pillars of accuracy, latency, and resource cost is challenging. In response to these challenges, we propose InfAdapter, which proactively selects a set of ML model variants with their resource allocations to meet latency SLO while maximizing an objective function composed of accuracy and cost. InfAdapter decreases SLO violation and costs up to 65% and 33%, respectively, compared to a popular industry autoscaler (Kubernetes Vertical Pod Autoscaler).

==> sections/batching_parallelism.tex <==
Apart from the size and the model variant used for the inference, batching and parallelism parameters are two other categories of parameters of ML services that can affect their performance and we need to analyze whether tuning those parameters at run-time can make a new opportunity to do the workload adaptation. We define bellow how these parameters work and the way they can affect the service performance:

\subsection{batching parameters}
There are usually two parameters used for dynamic batching of the requests on the ML services. The first one is the \textsc{maximum batch size}, which is a number to determine how many requests at most can be batched together to be given to the model and the second parameter is \textsc{maximum request delay}, which determines how long a request can be kept in a queue to wait for other requests for batching \cite{zhang2019mark, ali2020batch, tensorflow_serving_configuration, torchserve}. When any of these two parameters reach their maximum, the requests in the queue are batched and sent to the model for inference. The use of batching helps improve throughput and resource utilization when the underlying hardware can well parallel the execution of batches, As the case when hardware accelerators like GPUs are used.

\subsection{parallelism parameters}
TensorFlow Serving \cite{parallelism_tf} and TorchServe \cite{parallelism_torch} implement two thread pools, \textsc{intra\_op parallelism} and \textsc{inter\_op parallelism}, to better utilize CPU and gain performance improvement. Inter\_op parallelism defines the number of threads used for processing independent operations of inference requests in the server, while \textsc{intra\_op parallelism} defines the number of threads used for processing each individual inference operation of the model (like matrix multiplication). \textsc{Inter\_op parallelism} helps processing operations of multiple requests at the same time, thus improving the service throughput and \textsc{intra\_op parallelism} helps to process each operation of a request faster.

To have a better understanding of the impacts of batching and parallelism parameters, we did experiments picking some different options for them and finding the throughput-average\_latency relation; Starting the load from 1 QPS and gradually increasing the offered load, we find the saturation point for the service under the given configuration. All our experiments are done on a Kubernetes CPU cluster and the ML models are served by TensorFlow Serving. Figure \ref{fig:parameter-batch-saturation} shows the effect of batching along with parallelism parameters. Based on the observation, batching does not cause a negligible improvement on performance when the service is running on CPU, by comparing the best parallelism configuration in each figure which is the green plot. The purpose of batching is to utilize the hardware parallelism ability to process more requests at once, and since the parallelism degree of CPUs is far less than hardware accelerators like GPUs, batching is not much helpful. Another reason that we do not see much improvement here is that we are obtaining maximum parallelism degree and CPU utilization by just using the \textsc{inter\_op\_parallelism} thread pool, which helps to process multiple ML model operations of the requests at the same time. The reason that setting both \textsc{inter\_op\_parallelism} and \textsc{intra\_op\_parallelism} thread pools to the size of CPU (4 cores in this experiment) works not as well as setting \textsc{inter\_op\_parallelism} thread pool to the number of CPU cores and setting \textsc{intra\_op\_parallelism} thread pool to 1 (disabling it), is that the prior causes over-subscription, leading to service container CPU being throttled.

\begin{figure}[t]
\centering
\includegraphics[scale=0.2]{Figures/paralellism-batch-saturation.pdf}
\caption{Saturation throughput for \textsc{max\_batch\_sizes} of 1 (batching disabled), 4 and 16 under different parallelism configurations. Resnet50 with 4 CPU cores is used in this experiment.}
\label{fig:parameter-batch-saturation}
\end{figure}
